Online Convex Optimization Perspective for Learning from Dynamically Revealed Preferences

We study the problem of online learning (OL) from revealed preferences: a learner wishes to learn a non-strategic agent's private utility function through observing the agent's utility-maximizing actions in a changing environment. We adopt an online inverse optimization setup, where the learner observes a stream of agent's actions in an online fashion and the learning performance is measured by regret associated with a loss function. We first characterize a special but broad class of agent's utility functions, then utilize this structure in designing a new convex loss function. We establish that the regret with respect to our new loss function also bounds the regret with respect to all other usual loss functions in the literature. This allows us to design a flexible OL framework that enables a unified treatment of loss functions and supports a variety of online convex optimization algorithms. We demonstrate with theoretical and empirical evidence that our framework based on the new loss function (in particular online Mirror Descent) has significant advantages in terms of regret performance and solution time over other OL algorithms from the literature and bypasses the previous technical assumptions as well.

==> Def.tex <==
%%%
% Definitions conflicting with Alex's file: 
% I have commented these out in this file
%%%

%Colors
\def\crd{\color{red}}
\def\cbl{\color{blue}}
\def\cgr{\color{green}}
\def\cmg{\color{magenta}}
\def\ccy{\color{cyan}}
\def\cye{\color{yellow}}
\definecolor{gold}{rgb}{0.85,0.65,0}
%\colorlet{TepperRed}{red!70!black} 

%Shorthand
\newcommand{\wrt}{w.r.t.}
\def\iff{\text{if and only if}}
\def\WLOG{\text{Without loss of generality}}
\def\wLOG{\text{without loss of generality}}


%Equations, numbering, etc
\newcommand{\nin}{\noindent}
\newcommand{\nn}{\nonumber \\}
\renewcommand{\theequation}{\mbox{\arabic{equation}}}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}[1]{\label{#1}\end{eqnarray}}
\newcommand{\ese}{\end{eqnarray*}}
\newcommand{\bse}{\begin{eqnarray*}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\Bbb#1{{\bf #1}}
\def\eqnum#1{\eqno (#1)}
\def\fnote#1{\footnote}
%\newcommand{\epr}{\hfill\ensuremath{\Box}}
\newcommand{\epr}{\hfill\hbox{\hskip 4pt \vrule width 5pt height 6pt depth 1.5pt}\vspace{0.0cm}\par}
%\def\qed{$\Box$}
% \def\qed{\ \hfill$\square$\par\smallskip}


\def\ra{\rangle}
\def\la{\langle}
\def\ul{\underline}
%\def\*{{{\LARGE\bf $^*$}}}
%\def\P{{{\LARGE\bf $^+$}}}
%\def\PP{{{\LARGE\bf $^{++}$}}}

%Elementary functions
\newcommand{\floor}[1]{\ensuremath{\left\lfloor #1 \right\rfloor}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil #1 \right\rceil}}
\newcommand{\abs}[1]{\ensuremath{\left\lvert #1 \right\rvert}}
\DeclareMathOperator{\poly}{poly}
\newcommand{\by}{\times}
 
%Vector/matrix calculus
\newcommand{\norm}[1]{\ensuremath{\left\lVert #1 \right\rVert}}
\newcommand{\ip}[1]{\ensuremath{\left\langle #1 \right\rangle}}
\newcommand{\grad}{\ensuremath{\nabla}}

%P, NP, co-NP, etc.
\def\P{{\textsf\bf P\,}}
\def\NP{{\textsf\bf NP\,}}


%Letters in different typefaces
%\newcommand{\A}{\mathbb{A}}
\def\A{{\mathbb{A}}}
\def\B{{\mathbb{B}}}
\def\C{{\mathbb{C}}}
\def\D{{\mathbb{D}}}
\def\E{{\mathbb{E}}}
\def\F{{\mathbb{F}}}
\def\G{{\mathbb{G}}}
\def\H{{\mathbb{H}}}
\def\I{{\mathbb{I}}}
\def\J{{\mathbb{J}}}
\def\K{{\mathbb{K}}}
\def\L{{\mathbb{L}}}
\def\M{{\mathbb{M}}}
\def\N{{\mathbb{N}}}
\def\O{{\mathbb{O}}}
\def\P{{\mathbb{P}}}
\def\Q{{\mathbb{Q}}}
\def\R{{\mathbb{R}}}
\def\S{{\mathbb{S}}}
\def\T{{\mathbb{T}}}
\def\U{{\mathbb{U}}}
\def\V{{\mathbb{V}}}
\def\W{{\mathbb{W}}}
\def\X{{\mathbb{X}}}
\def\Y{{\mathbb{Y}}}
\def\Z{{\mathbb{Z}}}
\def\Le{{\mathbb{L}}}
\def\Se{{\mathbb{S}}}


\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

\newcommand{\CA}{\mathcal{A}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CD}{\mathcal{D}}
\newcommand{\CE}{\mathcal{E}}
\newcommand{\CF}{\mathcal{F}}
\newcommand{\CG}{\mathcal{G}}
\newcommand{\CH}{\mathcal{H}}
\newcommand{\CI}{\mathcal{I}}
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\CK}{\mathcal{K}}
\newcommand{\CL}{\mathcal{L}}
\newcommand{\CM}{\mathcal{M}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\CO}{\mathcal{O}}
\newcommand{\CP}{\mathcal{P}}
\newcommand{\CQ}{\mathcal{Q}}
\newcommand{\CR}{\mathcal{R}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CU}{\mathcal{U}}
\newcommand{\CV}{\mathcal{V}}
\newcommand{\CW}{\mathcal{W}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\CY}{\mathcal{Y}}
\newcommand{\CZ}{\mathcal{Z}}



\def\mones{{\mathbf{1}}}

\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}

\def\Ic{{\overline{I}}}

\def\e{\mathop{{\rm e}}}
%\def\i{{\mathop{z}}}
\def\nrm{\mathop{{\parallel}}}
\def\vrt{\mathop{\,\mid}\,}
\def\eqbd{\colon =}

%Optimization basics
\DeclareMathOperator{\Opt}{Opt}
\def\Argmin{\mathop{\rm Argmin}}
%\def\argmin{\mathop{\rm argmin}}
\def\Argmax{\mathop{\rm Argmax}}
%\def\argmax{{\mathop{\rm argmax}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%Saddle point and VI related
\DeclareMathOperator{\SadVal}{SV}
\DeclareMathOperator{\SV}{SV}
\DeclareMathOperator{\sad}{sad}
\newcommand{\VI}{VI}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\proj}{Proj}
\DeclareMathOperator{\Prox}{Prox}
\DeclareMathOperator{\Entr}{Entr}
\def\epsilonsad{{\epsilon_{\hbox{\scriptsize\rm sad}}}}
\def\epsilonsad{\epsilon_{\sad}}
\def\epsilonvi{\epsilon_{\hbox{\scriptsize VI}}}
\def\epsilonN{\epsilon_{\hbox{\scriptsize Nash}}}
\def\Sad{{\mathop{\rm Sad}}}
\def\Residual{\mathop{{\rm Residual}}}
\def\DualityGap{{\hbox{\rm DualityGap}}}
\newcommand{\dgf}{d.g.f.}



\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\sgn}{sign}
\DeclareMathOperator{\Supp}{supp}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Card}{Card}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\Size}{Size}
\DeclareMathOperator{\size}{Size}
\DeclareMathOperator{\Sz}{Size}
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\vol}{Vol}
\DeclareMathOperator{\Diam}{Diam}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\AvDiam}{AvDiam}
\DeclareMathOperator{\nnz}{nnz}
\DeclareMathOperator{\data}{data}
\DeclareMathOperator{\const}{const}

%Matrix related
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\rk}{rank}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Trace}{Trace}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\Det}{Det}
%\DeclareMathOperator{\det}{det}
\DeclareMathOperator{\Col}{Col}
\DeclareMathOperator{\Row}{Row}
\DeclareMathOperator{\Null}{null}
%\DeclareMathOperator{\null}{null}
\DeclareMathOperator{\nullity}{null}
%\DeclareMathOperator{\Ker}{Ker} %defined later in the "function related" section
\DeclareMathOperator{\Image}{Im}
\DeclareMathOperator{\Imm}{Im}
\DeclareMathOperator{\Range}{range}
\DeclareMathOperator{\range}{range}
\def\Arrow{{\hbox{\rm Arrow}}}
\def\Fr{{\hbox{\scriptsize Fr}}}
\def\Fro{\mathop{\hbox{\rm\scriptsize Fro}}}
\def\Spec{\mathop{\hbox{\rm\scriptsize Spec}}}


%Probability and distributions
\def\Prob{{\hbox{\rm Prob}}}
\def\Cov{{\hbox{\rm Cov}}}
\def\cov{{\hbox{\rm Cov}}}
\def\uniform{\mathop{\rm uniform}}
\DeclareMathOperator{\Uniform}{Uniform}
\DeclareMathOperator{\Geometric}{Geometric}
\DeclareMathOperator{\Poisson}{Poisson}
\DeclareMathOperator{\Var}{Var} %for variance
\DeclareMathOperator{\var}{Var} %for variance
\DeclareMathOperator{\CVaR}{CVaR}
\DeclareMathOperator{\KL}{KL}
\newcommand{\dist}{\sim}


%Topology related
\def\dim{\mathop{{\rm dim}\,}}
%\DeclareMathOperator{\dim}{dim}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\Lin}{Lin}
\DeclareMathOperator{\lin}{lin}
\DeclareMathOperator{\Aff}{aff}
\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\spann}{span}
%\DeclareMathOperator{\span}{Span} %Defining lowercase span clashes with some package options related to page layout and it is a bad idea.
\DeclareMathOperator{\intt}{int}
\DeclareMathOperator{\myint}{int}
\DeclareMathOperator{\inter}{int}
\DeclareMathOperator{\relint}{rel int} %rint %ri
\DeclareMathOperator{\rint}{rel int}
\DeclareMathOperator{\ri}{rel int}
\DeclareMathOperator{\partialri}{rel int}
%\def\partialri{\mathop{\partial_{\rm ri}}}
\DeclareMathOperator{\cl}{cl}
%\def\clsr{{\rm cl}}
\DeclareMathOperator{\bd}{bd}
\DeclareMathOperator{\rbd}{rbd}
\newcommand{\boundary}{\partial}


%Function related
\DeclareMathOperator{\Dom}{Dom}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\Epi}{Epi}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\Ker}{Ker}
%\DeclareMathOperator{\ker}{Ker}

%Convexity related
\DeclareMathOperator{\Conv}{Conv}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\co}{conv}
\DeclareMathOperator{\Cone}{Cone}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\cconv}{\overline{conv}}
\DeclareMathOperator{\clconv}{\overline{conv}}
\DeclareMathOperator{\clcone}{\overline{cone}}
\DeclareMathOperator{\ccvh}{\overline{conv}}
\DeclareMathOperator{\ccnh}{\overline{cone}}
\def\Ext{{\mathop{\rm Ext}}}
\def\ext{{\mathop{\rm ext}}}
\def\Extr{{\mathop{\rm Extr}}}
\def\extr{{\mathop{\rm extr}}}
\DeclareMathOperator{\Rec}{Rec}
\DeclareMathOperator{\rec}{rec}
\DeclareMathOperator{\apex}{apex}


\def\distt{\mathop{{\rm dist}}}
\def\log{\mathop{{\rm log}}}
\def\asin{{\hbox{\rm asin}}}
\def\Polar{{\mathop{{\rm Polar\,}}}}
\def\ch{{\mathop{\rm ch\,}}}
\def\arc{{\mathop{\rm arc\,}}}
\def\EllIn{{\mathop{\rm EllIn}}}
\def\GDA{{\rm \ ArD\ }}
\def\GDS{{\rm \ StD\ }}
\def\lev{{\mathop{\rm lev}}}


%Shapes etc.
\def\rdiamondsuit{{\color{red}$\diamondsuit$}}
\def\rclubsuit{{\color{red}$\clubsuit$}\ }
\def\rspadesuit{{\color{red}$\spadesuit$}\ }
\def\rbullet{{\color{red}$\bullet$}\ }
\def\rheartsuit{{\color{red}$\heartsuit$}}
\def\rArrow{{\color{red}$\Rightarrow$}\ }
\def\blacksquare{\hbox{\vrule width 4pt height 4pt depth 0pt}}
% square is actually a redefinition, this breaks the assumption and example environments
% \def\square{\hbox{\vrule\vbox{\hrule\phantom{o}\hrule}\vrule}} 


%Spacing, picture sizing related
\def\nr{\par \noindent}
\def\pn{\par\noindent}
\def\qr{\qquad\cr}
\def\fig{\epsfxsize=220pt\epsfysize=140pt\epsffile}
\def\mypictsmall{\epsfxsize=120pt\epsfysize=120pt\epsffile}
\def\mypictvsmall{\epsfxsize=90pt\epsfysize=90pt\epsffile}

\def\huh{\hbox{\vrule width 2pt height 8pt depth 2pt}}



\def\CE{\mathop{{\hbox{\sl CircEll}}}}
\def\CS{\mathop{{\hbox{\sl CircSimp}}}}
\def\IE{\mathop{{\hbox{\sl InscrEll}}}}
\def\Compl{\mathop{{\rm Compl}}}
\def\Accur{\mathop{{\rm Accur}}}
\def\mes{\mathop{{\rm mes}}}
\def\EllOut{\mathop{{\rm EllOut}}}
\def\Ell{\mathop{{\sl Ell}}}
\def\InnerRad{\mathop{{\rm InnerRad}}}
\def\Mom{\mathop{\rm Mom}}
\def\Loss{{\hbox{\rm Loss}}}


\def\bStnu{\bS^{\widetilde{\nu}}}
\def\bStnup{\bS^{\widetilde{\nu}}_+}




